Comparing Humans and Models on a Similar Scale: Towards Cognitive Gender Bias Evaluation in Coreference Resolution

Spurious correlations were found to be an important factor explaining model performance in various NLP tasks (e.g., gender or racial artifacts), often considered to be ''shortcuts'' to the actual task. However, humans tend to similarly make quick (and sometimes wrong) predictions based on societal and cognitive presuppositions. In this work we address the question: can we quantify the extent to which model biases reflect human behaviour? Answering this question will help shed light on model performance and provide meaningful comparisons against humans. We approach this question through the lens of the dual-process theory for human decision-making. This theory differentiates between an automatic unconscious (and sometimes biased) ''fast system'' and a ''slow system'', which when triggered may revisit earlier automatic reactions. We make several observations from two crowdsourcing experiments of gender bias in coreference resolution, using self-paced reading to study the ''fast'' system, and question answering to study the ''slow'' system under a constrained time setting. On real-world data humans make $\sim$3\% more gender-biased decisions compared to models, while on synthetic data models are $\sim$12\% more biased.

==> acl-ijcnlp2021-templates/acl.tex <==
% % This must be in the first 5 lines to tell arXiv to use pdfLaTeX, which is strongly recommended.
% \pdfoutput=1
% % In particular, the hyperref package requires pdfLaTeX in order to break URLs across lines.

% \documentclass[11pt]{article}

% % Remove the "review" option to generate the final version.
% \usepackage[review]{acl}

% % Standard package includes
% \usepackage{times}
% \usepackage{latexsym}

% % For proper rendering and hyphenation of words containing Latin characters (including in bib files)
% \usepackage[T1]{fontenc}
% % For Vietnamese characters
% % \usepackage[T5]{fontenc}
% % See https://www.latex-project.org/help/documentation/encguide.pdf for other character sets

% % This assumes your files are encoded as UTF8
% \usepackage[utf8]{inputenc}

% % This is not strictly necessary, and may be commented out,
% % but it will improve the layout of the manuscript,
% % and will typically save some space.
% \usepackage{microtype}

% % If the title and author information does not fit in the area allocated, uncomment the following
% %
% %\setlength\titlebox{<dim>}
% %
% % and set <dim> to something 5cm or larger.



% %
% % File acl2021.tex
% %
% %% Based on the style files for EMNLP 2020, which were
% %% Based on the style files for ACL 2020, which were
% %% Based on the style files for ACL 2018, NAACL 2018/19, which were
% %% Based on the style files for ACL-2015, with some improvements
% %%  taken from the NAACL-2016 style
% %% Based on the style files for ACL-2014, which were, in turn,
% %% based on ACL-2013, ACL-2012, ACL-2011, ACL-2010, ACL-IJCNLP-2009,
% %% EACL-2009, IJCNLP-2008...
% %% Based on the style files for EACL 2006 by 
% %%e.agirre@ehu.es or Sergi.Balari@uab.es
% %% and that of ACL 08 by Joakim Nivre and Noah Smith

% % \documentclass[11pt,a4paper]{article}
% % \usepackage[hyperref]{acl2021}
% % \usepackage{times}
% % \usepackage{latexsym}
% \usepackage{tikz}
% \renewcommand{\UrlFont}{\ttfamily\small}
% \usepackage{booktabs}
% %\usepackage{ulem}
% \usepackage{tabularx}
% \usepackage{graphicx}
% \usepackage{multirow}
% \graphicspath{{images/}}
% \usepackage{subcaption}
% \captionsetup{compatibility=false}



% % % This is not strictly necessary, and may be commented out,
% % % but it will improve the layout of the manuscript,
% % % and will typically save some space.
% % \usepackage{microtype}


% %% Local imports
% \usepackage[normalem]{ulem}
% \newcommand{\draftcomment}[3]{{\textcolor{#3}{[#1]#2}}}
% \newcommand{\gabisrw}[1]{\draftcomment{#1}{\textsc{gabi}}{purple}}
% \newcommand{\gabis}[1]{\draftcomment{#1}{\textsc{gabi}}{blue}}
% \newcommand{\gili}[1]{\draftcomment{#1}{\textsc{gili}}{red}}
% \newcommand{\gabisrep}[2]{\gabisrw{\sout{#1} #2}}
% \newcommand{\gabist}[1]{\gabisrw{\sout{#1}}}
% \newcommand{\LA}[0]{\ensuremath{\leftarrow}}
% %%

% %\aclfinalcopy % Uncomment this line for the final submission
% %\def\aclpaperid{***} %  Enter the acl Paper ID here

% %\setlength\titlebox{5cm}
% % You can expand the titlebox if you need extra space
% % to show all the authors. Please do not make the titlebox
% % smaller than 5cm (the original size); we will check this
% % in the camera-ready version and ask you to change it back.

% \newcommand\BibTeX{B\textsc{ib}\TeX}
% \newcommand{\winogender}[0]{Winogender}
% \newcommand{\winobias}[0]{WinoBias}
% \newcommand{\sys}[1]{\textit{System #1}}

% % If the title and author information does not fit in the area allocated, uncomment the following
% %
% %\setlength\titlebox{<dim>}
% %
% % and set <dim> to something 5cm or larger.

% \title{Comparing Humans and Models on a Similar Scale:\\
% Towards Cognitive Gender Bias Evaluation in Coreference Resolution

% }
% % Author information can be set in various styles:
% % For several authors from the same institution:
% % \author{Author 1 \and ... \and Author n \\
% %         Address line \\ ... \\ Address line}
% % if the names do not fit well on one line use
% %         Author 1 \\ {\bf Author 2} \\ ... \\ {\bf Author n} \\
% % For authors from different institutions:
% % \author{Author 1 \\ Address line \\  ... \\ Address line
% %         \And  ... \And
% %         Author n \\ Address line \\ ... \\ Address line}
% % To start a seperate ``row'' of authors use \AND, as in
% % \author{Author 1 \\ Address line \\  ... \\ Address line
% %         \AND
% %         Author 2 \\ Address line \\ ... \\ Address line \And
% %         Author 3 \\ Address line \\ ... \\ Address line}

% \author{First Author \\
%   Affiliation / Address line 1 \\
%   Affiliation / Address line 2 \\
%   Affiliation / Address line 3 \\
%   \texttt{email@domain} \\\And
%   Second Author \\
%   Affiliation / Address line 1 \\
%   Affiliation / Address line 2 \\
%   Affiliation / Address line 3 \\
%   \texttt{email@domain} \\}


% \date{}

% \begin{document}
% \maketitle
% \begin{abstract}
% \input{acl-ijcnlp2021-templates/sections/00_abstract}
% \end{abstract}

% \section{Introduction}
% \input{acl-ijcnlp2021-templates/sections/01_introduction}

% \section{Background}
% \input{acl-ijcnlp2021-templates/sections/02_background}

% \section{Working Definitions}
% \label{sec:key-definitions}
% \input{acl-ijcnlp2021-templates/sections/03_key_definitions}

% \section{Experiments}
% \label{sec:experiments}
% \input{acl-ijcnlp2021-templates/sections/05_experiments}

% \section{Results}
% \label{sec:results}
% \input{acl-ijcnlp2021-templates/sections/06_results}

% \section{Coreference Models Case Study}
% \label{sec:case-study}
% \input{acl-ijcnlp2021-templates/sections/models_case_study}

% \section{Ways Forward}
% \input{acl-ijcnlp2021-templates/sections/ways_forward}

% \section{Discussion}
% \input{acl-ijcnlp2021-templates/sections/07_discussion}

% \section{Limitations}
% \input{acl-ijcnlp2021-templates/sections/08_limitations}

% \bibliographystyle{acl_natbib}
% \bibliography{anthology,acl2021}
% % \bibliography{anthology,custom}

% \appendix

% \section{Appendix}
% \label{sec:appendix}

% \input{acl-ijcnlp2021-templates/sections/appendix}

% \end{document}


==> acl-ijcnlp2021-templates/figures/MAZE_dist_figure.tex <==
% \begin{figure}[]
% \centering
% \begin{subfigure}{0.45\columnwidth}
%   \includegraphics[width=\columnwidth]{acl-ijcnlp2021-templates/images/Wino_distances_std.png}
%   \caption{}
%   \label{fig:MAZE-dist-wino}
% \end{subfigure}
% \begin{subfigure}{0.45\columnwidth}
%   \includegraphics[width=\columnwidth]{acl-ijcnlp2021-templates/images/BUG_distances_std.png}
%   \caption{}
%   \label{fig:MAZE-dist-BUG}
% \end{subfigure}
% \caption{}
% \label{fig:MAZE-distances}
% \end{figure}

\begin{figure}
\centering
 \includegraphics[width=\columnwidth]{acl-ijcnlp2021-templates/images/distances_std.png}
 \caption{Mean response time to distinguish the pronoun in the MAZE task across the different participants, as a function of the distance (in words) between the pronoun and its antecedent. The vertical lines present an adjusted variance:~$\pm$ mean$(|RT-$mean$(RT)|)$, where $RT$ is a participant response time.} 
 \label{fig:MAZE-dist}
\end{figure}

==> acl-ijcnlp2021-templates/sections/00_abstract_new.tex <==

% models achieve impressive results over different language tasks

% however it has recently shown that it is gained by ``shortcuts'': exploiting statistical correlations in the data rather then solving the actual task, also known as spurious correlations.

% It has also shown that models rely on social biases  (gender, race, etc.) during inference, which can be a result of either (a) spurious correlations, or (b) models reflecting human trait i.e., reflecting human biases. 

% In this work, we tease those two apart, by putting humans and models on the same scale. We want to learn what causes model gender bias, since each cause requires a different approach for mitigating model biases. If we find it is spurious correlations, debiasing may focus on improving dataset collection. But for the latter, debiasing is more complicated. Learning human behaviour is necessary in some cases, e.g., for commonsense reasoning and handling missing information. So if we find that model biases are caused by reflecting human biases, debiasing may focus on models training procedure, by teaching models to reflect the desired human traits, without learning the harmful ones.

==> acl-ijcnlp2021-templates/sections/04_motivation.tex <==

We note  that it is common practice to compare model level accuracy on downstream task performance, e.g., in question answering, summarization, or natural language inference.\footnote{E.g., in leaderboards such as \url{https://leaderboard.allenai.org/}} Here we advocate that gender bias should similarly be compared against human-level performance on similar metrics. This can aid in identifying whether models amplify the bias found in the data (in case they rely on bias more than humans do), mitigate it (in case they rely on it less), or simply mirror it (if their gender bias is similar to humans').
These comparisons can shed light on the way forward towards less gender-biased models. For example, if gender bias is amplified in models, then perhaps focus should be put on better modelling, while if it is mitigated or mirrored, then perhaps the bottleneck for less biased models lies in more balanced datasets.


%(0) probing models
In this Work we will focus on the coreference resolution downstream task. As shown in Figure~\ref{fig:fig1}, our work follows two parallel tracks, one for model evaluation and one for human evaluation, to get both humans and models results over the coreference resolution task on the same scale. Previous work presented deterministic probing~\citep{clark-etal-2019-bert, sorodoc-etal-2020-probing}, which is isolating the different features that are expected to affect models' performance, and test each of them separately. Some well known features that affect coreference resolution performance are structural factors such as the distance between the pronoun and the entity~\citep{bengtson-roth-2008-understanding} and the number of pronouns and entities in the sentence~\citep{zhou-choi-2018-exist}, morphosyntactic factors such as grammatical constraints~\citep{sorodoc-etal-2020-probing}, semantic factors such as referential
information~\citep{sorodoc-etal-2020-probing} and the semantic relation between the entities such as gender agreement, number agreement, is one entity acronym of the other, type match and more (see~\citealp{recasens2009deeper} for a comprehensive list of features). So for the model evaluation track in this work, we will probe a small subset of features that effect model coreference resolution performance.

%(1) probing for humans is hard, so to assess human biases we turn to the broad literature on psycholinguistics, and specifically focus on the two systems hypothesis.
Ideally, we would like to ``probe'' humans on similar metrics. However, similar deterministic probing of human behaviour seems hard. For example, \citet{Rogers2011TheRO} showed that the level of dopamine and serotonin activity plays a significant role in humans' desicion making process, which is a factor that is hard to control when trying to isolate other factors effecting humans behaviour. So for the human evaluation track in our work, we turn to the broad literature on psycholinguistics, that widely covers the gender bias phenomenon for humans over different linguistic tasks. For example,~\citet{osterhout1997brain} recorded event-related brain potentials (ERPs, brain response to specific events or stimuli), for reading sentences with reflexive pronouns (``himself''/``herself''), for both anti-stereotype and pro-stereotype sentences.~\citet{kennison2003comprehending} collected results of the effect of gender stereotypes over language comprehension, by measuring reading times of different parts in a sentence.~\citet{duffy2004violating} collected information regarding eye movements, and especially fixation times, for sentences with gender stereotype professions, and a reflexive pronoun. For the humans evaluation track as shown in Figure~\ref{fig:fig1}, in this work we assessing human biases by specifically focus on the dual-process theory~\citep{evans2008dual, kahneman2011thinking}.

%(2) This approach posits that human cognition ...
This theory posits for two cognitive systems participating in humans' decision making process. \sys{1} is fast, associative and automatic, while \sys{2} is slower, controlled and conscious. For example, orient to the source of a sudden sound or answering ``2+2=?'' only involves \sys{1}, while filling out a tax form or checking the validity of a complex logical argument invoke \sys{2}~\citep{kahneman2011thinking}. 

% link between dual process to NLP probing
We link between the dual-process theory and the NLP literature on probing model performance, by assigning each probing mechanism to one of the two systems. In particular, We associate syntactic probes (e.g, word distance) with \sys{1}, since these probes are immediate and does not require analysis and comprehension, while we associate more semantic probes with \sys{2} (e.g., the semantic relation between the entities), as they require humans for more a complex analysis.


%(3) Following this approach we propose that human evaluation metrics target each of the systems to capture both immediate responses, as well as ... (4) In particular, we develop two evaluation methods which follow this methodology.
Following this approach we propose human evaluation metrics that target each of the systems to capture both immediate responses (\sys{1}), as well as more complex and processed responses (\sys{2}).
% (5) First, we propose eye tracking measurements as a proxy for \sys{1}, as it depends on subconscious decision making (here we should be careful and give some citation). In Section ... we leverage self-pace reading architecture to approximate eye-tracking and propose metrics to quantify how gender bias may manifest within it.
First, we propose eye tracking measurements as a proxy for \sys{1}, as eye-movements during reading has shown to be unconscious~\citep{rayner1998eye,rayner2009eye,miller2013unraveling}. In Section~\ref{sec:maze-experiment} we leverage self-pace reading architecture to approximate eye-tracking and propose metrics to quantify how gender bias may manifest within it.
%(6) Second, we propose question answering as a proxy for evaluating \sys{2}, as it requires more involved processing which is likely to invoke this decision making system (again, be careful and look for citations.
Second, we propose question answering as a proxy for evaluating \sys{2}, as it requires comprehension, that is considered a cognitive process that requires resources for finding relations and using long-term memory~\citep{wang2003cognitive}, which is likely to invoke \sys{2}.



==> acl-ijcnlp2021-templates/sections/04_motivation_old.tex <==

As presented in Section~\ref{sec:key-definitions}, both models and humans tend to over-rely on societal gender biases.

% models are gender biased (moved to gender bias def)
Previous studies showed that NLP state-of-the-art models are gender biased in different NLP tasks such as coreference resolution~\citep{rudinger-etal-2018-gender, zhao-etal-2018-gender}, machine translation~\citep{stanovsky-etal-2019-evaluating}, named entity recognition~\citep{mehrabi2020man}, relation extraction~\citep{gaut-etal-2020-towards}, and more (see~\citealp{sun-etal-2019-mitigating} for a comprehensive review). 

\gabisrw{We note  that it is common practice to compare model level accuracy on downstream task performance, e.g., in question answering, summarization, or natural language inference.\footnote{E.g., in leaderboards such as \url{https://leaderboard.allenai.org/}} Here we advocate that gender bias should similarly be compared against human-level performance on similar metrics. This can aid in identifying whether models amplify the bias found in the data (in case they rely on bias more than humans do), mitigate it (in case they rely on it less), or simply mirror it (if their gender bias is similar to humans').
These comparisons can shed light on the way forward towards less gender-biased models. For example, if gender bias is amplified in models, then perhaps focus should be put on better modelling, while if it is mitigated or mirrored, then perhaps the bottleneck for less biased models lies in more balanced datasets.}\gabis{\LA I think that something along this lines can appear here or in the intro. What do you think? If this looks good to you, then I think that a logical flow can be the one I suggest below. If this looks good to you, then maybe we can restructure what we already have around this flow? 
(1) To assess human biases we turn to the broad literature on psycholinguistics, and specifically focus on the two systems hypothesis.
(2) This approach posits that human cognition ...
(3) Following this approach we propose that human evaluation metrics target each of the systems to capture both immediate responses, as well as ...
(4) In particular, we develop two evaluation methods which follow this methodology. 
(5) First, we propose eye tracking measurements as a proxy for system 1, as it depdends on subconscious decision making (here we should be careful and give some citation). In Section ... we leverage self-pace reading architecture to approximate eye-tracking and propose metrics to quantify how gender bias may manifest within it.
(6) Second, we propose question answering as a proxy for evaluating system 2, as it requires more involved processing which is likely to invoke this decision making system (again, be careful and look for citations.
} 

% gender bias evaluation in models today
So far, the common practice in comparing NLP models to human performance over gender bias has been driven by accuracy measurement, such as precision or recall on pro-stereotype versus anti-stereotype sentences (\citealp{zhao-etal-2018-gender, stanovsky-etal-2019-evaluating, cho-etal-2019-measuring, sharma2021evaluating, levy-etal-2021-collecting-large}, inter alia). 

% put humans and models on the same scale
In this work, we attempt to compare human and machine gender bias on equal footing, and find under what conditions humans will perform similarly to current state-of-the-art models in terms of gender bias.

% defining methodology
Particularly, we explore time-based limitations on two cognitive tasks - question answering (QA) and self-paced reading. For both tasks we applied modifications in the setup, such as limiting the given time to complete the task, to control the difficulty of the task. We then measured the differences in performances on anti-stereotype and pro-stereotype sentences, as a results of the setup modifications, and used the difference as a measure for gender bias.\gili{The last sentence is more describing QA and not MAZE}

% methods relates to the 2 systems
We believe that the two different tasks applies evaluation over two different humans' decision making cognitive systems, according to psychology . This theory claims for two cognitive systems participating in humans' decision making process. System 1 is fast, associative and automatic, while system 2 is slower, controlled and conscious. A detailed explanation regarding the experiments tasks and their relation to the dual-process theories is presented in Section~\ref{sec:experiments}.

% reasoning for comparing humans and models
Since NLP models attempt to understand humans' language, we believe that the evaluation of models can be improved if it would be driven more by comparison to humans. 
% why using psycoliguistic to compare + example
This comparison can be improved with deeper understanding of humans' cognitive processes for the different linguistic tasks, which can benefit from a combined research with psycho-linguistic researchers. 
An example for such combined research was presented in~\citet{wilcox2021targeted}, that compared humans and NLP models over their behaviour around critical region for comprehension of a sentence. The time humans spent reading the critical region was compared to the model's usage of the critical region for its answer. This work tries to put humans and models on the same scale, and builds a measurement for models that has not been shown before. 

% psycholiguistic examples for gender bias testing
As far as we now, no such combined work has measured the gender bias phenomenon, though a lot of data have been collected by psycho-linguistic researchers regarding the effect of gender stereotype information over different linguistic tasks and different humans' cognitive processes. For example,~\citet{osterhout1997brain} recorded event-related brain potentials (ERPs, brain response to specific events or stimuli), for reading sentences with reflexive pronouns (``himself''/``herself''), for both anti-stereotype and pro-stereotype sentences.~\citet{kennison2003comprehending} collected results of the effect of gender stereotypes over language comprehension, by measuring reading times of different parts in a sentence.~\citet{duffy2004violating} collected information regarding eye movements, and especially fixation times, for sentences with gender stereotype professions, and a reflexive pronoun. All of these can be used for a comprehensive comparison between models and humans gender bias, that has not been shown so far, to better understand the gaps between humans and models, and to derive new methods for improving NLP models.

% present models - moved to background
In parallel to running the humans evaluations, in our work we also tested the performance of two coreference resolution state-of-the-art models: (1) spanBERT~\citep{joshi-etal-2020-spanbert}. (2) Lightweight model without span representations, presented by~\citet{kirstain-etal-2021-coreference}.

% probing models
A common way to asses the quality of a coreference resolution model is through deterministic  probing~\citep{clark-etal-2019-bert, sorodoc-etal-2020-probing}. That is, isolate the different features that are expected to affect models' performance, and test each of them separately. Some well known features that affect coreference resolution performance are structural factors such as the distance between the pronoun and the entity~\citep{bengtson-roth-2008-understanding} and the number of pronouns and entities in the sentence~\citep{zhou-choi-2018-exist}, morphosyntactic factors such as grammatical constraints~\citep{sorodoc-etal-2020-probing}, semantic factors such as referential
information~\citep{sorodoc-etal-2020-probing} and the semantic relation between the entities such as gender agreement, number agreement, is one entity acronym of the other, type match and more (see~\citealp{recasens2009deeper} for a comprehensive list of features).

% probing for humans is hard, so we use the 2 systems. 
Applying the same probing over humans is a desideratum, but since it is hard, in the following sections we suggest two methods to measure humans' performance.  Each one aims to isolates a different cognitive process, according to the dual-process theory. We suggest that each cognitive process is linked to a subset of the features that effect models, which their joint effect over humans can be captured through that cognitive process. We will compare each cognitive process results for humans with the effect of its matching subset of features for models. System 1 is able to capture the effect of non-conscious features that does not require additional processing, such as the distance between the entity and the pronoun and the amount of antecedents in a sentence. System 2 is aimed to capture the effect of features that require a deeper analysis of the sentence, such as the semantic relation between the entities.

In following sections we find that these metrics better surface biases in human annotations on levels similar to models, in certain scenarios, in comparison to previously suggested metrics. 

%~\citet{malmaud-etal-2020-bridging} collected a large eye-tracking dataset for multiple choice reading comprehension task for humans. The resulted dataset can be used to evaluate models over the same sentences, analyzing models mistake versus humans eye movement behaviour. This dataset can also be used for improving models, by taking humans fixation points and emphasize them in the input for training models.


==> acl-ijcnlp2021-templates/sections/07_discussion.tex <==

We presented a first evaluation of human versus model biases in the context of gender bias in coreference resolution. Comparable biases arise in humans (although on a smaller scale), indicating that the data artifacts model pick up are reflecting real-world human behavior, and debiasing might benefit from  modelling solutions rather than more balanced datasets. In addition, our evaluation framework can be used to test future coreference resolution models. 

Our work opens the door for many promising avenues of future work, including (1) experimenting with both \sys{1} and \sys{2} in a single task; (2) finding better distractors for the self-paced reading task; and (3) experimenting QA on a more gradual fraction of reading pace. (4) Comparing \sys{1} with the few first layers of the network.

% \paragraph{Total performance trend of \sys{2}}We conclude that for the synthetic sentences in \winobias{} and \winogender{} datasets, time reduction indeed surface the gender bias phenomena, but there is a fraction between $0.5$ to $0.25$ that is the lower bound for examining it.

% \paragraph{The fact that QA captures gender bias while MAZE doesn’t, indicates that system1 does suffer from gender bias, and MAZE is just not good enough to capture it}

==> acl-ijcnlp2021-templates/sections/ethics_statement.tex <==

Before running the human subject experiments, we completed the CITI program course ``Social \& Behavioral Research - Basic/Refresher'', following our institution's requirements.\footnote{\url{https://about.citiprogram.org/course/human-subjects-research-social-behavioral-educational-sbe-refresher-1/}}

As for our annotators, participants were anonymous and no personal data was collected by us. All participants consented to the task, after they were able to see detailed guidelines regarding what they are required to do. See Figure~\ref{fig:instructions} in the Appendix for an example instructions shown before our qualification task.

==> acl-ijcnlp2021-templates/sections/related_work.tex <==
https://arxiv.org/pdf/2111.07997.pdf
- Roger's latest gender bias
- the work that compare humans fixation times and models weights over parts of the sentence
https://aclanthology.org/2021.eacl-main.137.pdf

Top Hope:

Cognitive Biases in Crowdsourcing http://brown.edu/Research/AI/files/pubs/wsdm18.pdf

Eye Gaze and Self-attention: How Humans and Transformers Attend Words in Sentences https://aclanthology.org/2022.cmcl-1.9/


% Previous studies showed that NLP state-of-the-art models are gender biased in different NLP tasks such as coreference resolution~\citep{rudinger-etal-2018-gender, zhao-etal-2018-gender}, machine translation~\citep{stanovsky-etal-2019-evaluating}, named entity recognition~\citep{mehrabi2020man}, relation extraction~\citep{gaut-etal-2020-towards}, and more (see~\citealp{sun-etal-2019-mitigating} for a comprehensive review).
% Humans, however, are also susceptible to relying on this kind of gender bias~\citep{osterhout1997brain,kennison2003comprehending,duffy2004violating}. For example,~\citet{von2020implicit} tested participants on three different textual tasks (belief estimation, text completion, and self-paced reading) regarding the gender of ``president'' and ``prime-minister'' entities in text during elections campaigns. They showed that even in cases where the participants expected that the female candidate will win the election, they were still biased towards male president and prime-minister in the comprehension and text generation tasks.

==> acl-ijcnlp2021-templates/sections/ways_forward.tex <==
%\gabis{I felt like we used the paragraph format a lot, so I removed it here}

Our work opens the door for many promising avenues of future work, including (1) experimenting with both \sys{1} and \sys{2} in a single task; (2) finding better distractors for the self-paced reading task; (3) experimenting QA on a more gradual fraction of reading pace.



First, it is interesting to combine the suggested methods in this paper to better understand the interactions between \sys{1} and \sys{2}.
For instance, this can done by asking participants to perform more conscious tasks when reaching the last word in the sentence in the self-paced reading task, e.g., answer gender question about it.
% MAZE might becoming a highly technical task after number of iterations, so asking participants to reconstruct the sentence can possibly cause more focus on the sentence meaning, thus more focus on stereotypical relations between entities when distinguishing the next word. 
This will likely invoke \sys{2} in a task that is mainly focused around \sys{1}, and
test both systems in the same task.


Another axis to explore is the effect  that different distractors would have on our results. While A-maze chooses distractors from language models, it may be that a different approach would surface human gender bias more accurately.


% It can be interesting to check the effect of the presented distractors, over MAZE ability to surface gender bias. Different heuristics to choose a distractor for the pronoun, as well as using different language models to automatically generate distractors, might show different impact over gender bias occurrence.

Finally, our choice of fractions for the reading times ($\alpha \in \{0.25, 0.5, 0.75\}$) may be rather coarse. Instead, developing a gradual approach may better reflect human gender bias with finer detail.   


% The evaluation we suggest in this paper address only 4 time fraction ranges (0-0.25, 0.25-0.5, 0.5-0.75, 0.75-1). These ranges seem wide, so an improvement would be to annotate more data over different baseline time fractions in order to achieve narrower and more precise ranges.


%\gabis{I removed two directions here - larger scale I suggest to put in limitations, and I'm not sure I understand the second one}
% \paragraph{Run on larger scale.}
% All human evaluations we show in this paper are only correct for our specific group of participants. Enlarging the number of participants, as well as their diversity, can improve the suggested metrics, as it will improve their robustness to different societal biases that might effect the results.

% \paragraph{Investigate more deeply models spurious correlations.}
% In this paper we mostly focus on investigating human biases, and imply them to metrics that are comparable to models. A future interesting work can be the other direction, which is thoroughly investigate models spurious correlations that increase gender bias, and use them to compare to known human evaluations.


==> acl-ijcnlp2021-templates/tables/MAZE_total_performance_table.tex <==

\begin{table}[ht]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}cllll@{}}
\toprule
\multicolumn{1}{l}{Dataset}                                                        & Category       & \#Correct & \#Total & Success rate \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}winogender\\ +\\ winobias\end{tabular}} & pro-stereotype & 1274      & 1283    & 0.993        \\
                     & anti-stereotype & 1264 & 1283 & 0.985 \\
                     & neutral         & 264  & 268  & 0.985 \\
                     & pronoun-neutral & 141  & 143  & 0.986 \\ \midrule
\multirow{3}{*}{BUG} & pro-stereotype  & 1350 & 1383 & 0.976 \\
                     & anti-stereotype & 1152 & 1184 & 0.973 \\
                     & neutral         & 175  & 183  & 0.956 \\ \bottomrule
\end{tabular}%
}
\caption{Total performance over distinguishing the next word from a distractor, where the correct next word is the pronoun. \gili{remove?}}
\label{tab:MAZE-toal-performance}
\end{table}

==> acl-ijcnlp2021-templates/tables/QA_total_performance.tex <==

\begin{table}[ht]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}l|ll|ll@{}}
\toprule
 &
  \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}winogender\\ +\\ winobias\end{tabular}} &
  \multicolumn{2}{c}{BUG} \\ \cmidrule(l){2-5} 
\begin{tabular}[c]{@{}l@{}}fraction of\\ baseline time\end{tabular} &
  fillers &
  total &
  fillers &
  total \\ \midrule
0.75 & 80.46\% & 84.28\% & 62.62\% & 73.89\% \\
0.5  & 81.2\%  & 83.81\% & 60.52\% & 71.46\% \\
0.25 & 77.3\%  & 75.92\% & 60.41\% & 69.74\% \\ \bottomrule
\end{tabular}%
}
\caption{QA experiment aggregated performance. `fillers' stands for performance over fillers questions, as presented in Section~\ref{sec:QA-experiment}. `total' stands for aggregated performance over all types of sentences, including all different stereotype signals (pro, anti, neutral) and filler questions. Relatively low total performance is a result of low performance over filler questions, which was found out to be a results of the qa-srl model's mistakes, and not actual participants' mistakes.\gili{remove?}}
\label{tab:QA-total-performance}
\end{table}

==> acl-ijcnlp2021-templates/tables/datasets_length_table.tex <==

\begin{table}[h]
\centering
\begin{tabular}{@{}l|ll@{}}
\toprule
                           & \multicolumn{2}{c}{Sentence length} \\
                           & average.             & std.             \\ \midrule
\winobias   & 14.0             & 2.24             \\
\winogender & 15.66            & 3.13             \\
BUG                        & 27.39            & 12.07            \\ \bottomrule
\end{tabular}
\caption{The average length of a sentence in the dataset, and its standard deviation.}
\label{tab:datasets-avg}
\end{table}

==> main.tex <==
\pdfoutput=1
\input{CogSci_Template}
